INPROVF: Leveraging Large Language Models to Repair High-level Robot Controllers from Assumption Violations

This paper presents INPROVF, an automatic framework that combines large language models (LLMs) and formal methods to speed up the repair process of high-level robot controllers. Previous approaches based solely on formal methods are computationally expensive and cannot scale to large state spaces. In contrast, INPROVF uses LLMs to generate repair candidates, and formal methods to verify their correctness. To improve the quality of these candidates, our framework first translates the symbolic representations of the environment and controllers into natural language descriptions. If a candidate fails the verification, INPROVF provides feedback on potential unsafe behaviors or unsatisfied tasks, and iteratively prompts LLMs to generate improved solutions. We demonstrate the effectiveness of INPROVF through 12 violations with various workspaces, tasks, and state space sizes.

==> figures/casestudy.tex <==
\begin{figure*}[t]
  \centering
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Left Column
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[t]{0.496\textwidth}
  \vspace{0pt}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Abstraction informalization prompt
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{tcolorbox}[
      colback=blue!5!white,      % first color (blue)
      colframe=blue!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
    \scriptsize\textbf{A. Abstraction informalization prompt.} \\%\\[1mm]
    % \textbf{System prompt:}
You are a researcher in robotics and an expert in formal methods for robotics.
% \textbf{User prompt:}
% \vspace{-1.5em}
You are given an abstraction that contains a set of input propositions $\inp$, 
a physical state space $\ps \subseteq R^n$, 
and a grounding function $\grounding: \inp \to 2^\ps$ that maps each input proposition to a set of physical states. 
You are asked to explain the physical meaning of the input propositions.

\# Input propositions: 
\textbf{\textless Inserted input propositions $\inp$ \textgreater}

\# Grounding: 
\textbf{\textless Inserted grounding function $\grounding$ \textgreater}

Please only provide a concise, general explanation covering all input propositions' physical meaning. Do not provide any examples.

\textbf{\textless Informalized abstraction to be returned here\textgreater}
    \end{tcolorbox}
    \vspace{-1.5em}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Informalized Abstraction
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{tcolorbox}[
      colback=red!5,       % second color (red)
      colframe=red!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
    \scriptsize\textbf{B. Example informalized abstraction description from \gls{llms}.} \\%\\[1mm]
    Each input proposition $\varol{o}{r}$ represents the condition that object $o$ is located within region $r$. The grounding function $\grounding$ maps each proposition $\varol{o}{r}$ to the set of physical states where the pose of object $o$ is in region $r$. The proposition $\varol{\textrm{empty}}{}$ signifies the status of the cup, indicating whether it is empty.
    \end{tcolorbox}
\vspace{-1.5em}
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Strategy informalization prompt
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{tcolorbox}[
      colback=blue!5!white,      % first color (blue)
      colframe=blue!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
    \scriptsize\textbf{C. Strategy informalization prompt.} \\%\\[1mm]
    You are a researcher in robotics and an expert in formal methods for robotics.
You are given an abstraction of the environment, a set of robot skills, a GR(1) specification, and its corresponding synthesized strategy. You are asked to describe the behavior of the strategy. I will first give an example of a strategy, its behavior description, and its explanation. Then, I will ask you to describe the behavior of a different strategy.

\# Example: \textbf{\textless Inserted strategy informalization example
$(\strategy^1, \strategydescription^1)$. 
See Fig.~\ref{fig:inform_example}A for the exact text \textgreater}
% \# Example: \\
% \#\# Input propositions: 
% $["a"]$\\
% \#\# Output propositions: 
% $["b"]$\\
% \#\# Task specification: 
% $a \to b \land \square \lozenge (a\to b) \land \square \lozenge (\neg a\to \neg b)$\\
% \#\# Strategy:
% \{"nodes": \{"0": \{"rank": 0, "state": ["a"], "trans": [1, 2]\}, "1": \{"rank": 0, "state": [], "trans": [1, 0]\}, "2": \{"rank": 0, "state": ["a", "b"], "trans": [1, 0]\}\}\}\\
% \#\# Behavior:
% Initially, the input 'a' is true and the output 'b' is false. If 'a' remains true, 'b' turns on and off repeatedly. While 'a' becomes false, 'b' remains false.\\
% \#\# Explanation:
% "Initially, the input 'a' is true and the output 'b' is false" corresponds to node 0. "If 'a' remains true, 'b' turns on and off repeatedly" corresponds to the transitions between node 0 and node 2. "While 'a' becomes false, 'b' remains false" corresponds to the transitions from node 0 and node 2 to node 1 and self-transitions to node 1.

\# Problem:
Now, I will ask you to describe the behavior of a different strategy. You are given: (1) an abstraction of the physical workspace and objects in the workspace, (2) a set of robot skills, (3) a task specification, and (4) a synthesized robot controller.

\#\# Input propositions:
\textbf{\textless Inserted inputs $\inp$ and informalized abstraction\textgreater}

\#\# Output propositions:
\textbf{\textless Inserted output propositions $\out$\textgreater}

\#\# Task specification:
We use the \gls{gr1} fragment of Linear Temporal Logic to encode the task specification. The task specification is given in the following JSON file:
\textbf{\textless Inserted task specification $\spectask$\textgreater}

\#\# Strategy:
We represent the robot strategy synthesized from the specification as a finite state automaton. 
For each node, 'rank' represents which liveness goal the node is trying to satisfy, 'state' represents the value of each variable in the state, in the order of the field 'variables', and 'trans' represents the possible successor states. 
The strategy is in the JSON file:
\textbf{\textless Inserted strategy $\strategy$\textgreater}

Please describe the behavior of the synthesized strategy only. Do not provide any explanation:
\textbf{\textless Informalized strategy behavior to be returned here\textgreater}
    \end{tcolorbox}
\vspace{-1.5em}
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Informalized Strategy
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \begin{tcolorbox}[
      colback=red!5,       % second color (red)
      colframe=red!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
    \scriptsize\textbf{D. Example informalized strategy behavior from \gls{llms}.} \\%\\[1mm]
    The synthesized strategy behaves as follows:
Initially, the robot's base is at position $x_4$, the cup is at location $t_2$, the block is at location $t_1$, the cone is at $x_3$, the plate is at $t_0$, and the cup is empty.
%
When the cup becomes not empty, the robot executes skill$_4$ to pick up the block from $t_1$ and then skill$_7$ to place the block at $t_3$. Next, the robot uses skill$_2$ to pick up the cup from $t_2$. It then executes skill$_1$ to move from $x_4$ via $x_2$ to $x_0$ while holding the cup. At $x_0$, the robot uses skill$_6$ to place the cup on the table.
%
When the cup becomes empty again, the robot executes skill$_3$ to pick up the cup from the table. It then uses skill$_0$ to move from $x_0$ via $x_2$ to $x_4$ while holding the cup. At $x_4$, the robot executes skill$_5$ to place the cup back at $t_2$.
    \end{tcolorbox}
\vspace{-1.5em}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % New skills that fail liveness analysis
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{tcolorbox}[
      colback=red!5,       % second color (red)
      colframe=red!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
\scriptsize\textbf{G. Example new skill candidates that cannot satisfy liveness constraints.}
\begin{lstlisting}[basicstyle=\scriptsize]
```JSON
{   "new_skill_0": [
        [["p_base_x2", "p_cup_ee", "p_block_k3"], 
        [["p_base_x4", "p_cup_ee", "p_block_k3"]]]]}
```
\end{lstlisting}
\textbf{Feedback from liveness analysis}: 
The new skills cannot satisfy the liveness goals 
$\square\lozenge (\varol{\textrm{empty}}{} \to \varol{\textrm{cup}}{t_2})$.
% ( empty $\to$ p\_cup\_k2 ).
% "!(p\_base\_x3' \& p\_cone\_x3')"
    \end{tcolorbox}
    
  \end{minipage}
  %%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%
  \hfill
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Right Column
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[t]{0.496\textwidth}\vspace{0pt}
    
        \begin{tcolorbox}[
      colback=blue!5!white,      % first color (blue)
      colframe=blue!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
    \scriptsize\textbf{E. Repair prompt.} \\%\\[1mm]
    You are a researcher in robotics and an expert in formal methods for robotics.
% \textbf{User prompt:}
You are given: (1) an abstraction of the physical workspace and objects in the workspace, (2) a set of robot skills, (3) a task specification, (4) the original behavior of the synthesized strategy, and (5) a violated observation during the robot execution.
You are asked to provide a set of new skills that along with the original skills can allow the robot to recover from the violation and satisfy the task specification.

\# Abstraction:\\
\#\# Input propositions:
\textbf{\textless Inserted inputs $\inp$ and informalized abstraction\textgreater}

\#\# Output propositions:
\textbf{\textless Inserted output propositions $\out$\textgreater}

\# Task specification:\\
We use the \gls{gr1} fragment of Linear Temporal Logic to encode the task specification. The task specification is given in the following JSON file:
\textbf{\textless Inserted task specification $\spectask$\textgreater}

\# Strategy behavior:
\textbf{\textless Inserted informalized strategy behavior\textgreater}

\# Assumption Violation:
During the robot execution, we detect that an observed transition violates some environment safety assumptions.

\#\# The violated observation is in the following JSON file:\\
\textbf{\textless Inserted assumption violation $t=(\inpstate, \outstate, \inpstateprime)$\textgreater}

\#\# The violated environment safety assumptions are as follows:\\
\textbf{\textless Inserted violated assumptions $\envsafetyvio$ \textgreater}

\# Returns:
After the assumption violation, we relax the violated assumption to include the observed violation transition. You are asked to provide a set of new skills that, along with the original skills, allow the robot to continue satisfying the task after the assumption violation.
Please respond with new skills only in the following format:
\begin{lstlisting}[basicstyle=\scriptsize]
```JSON
{  "new_skill_0": [
            [ <PRECONDITION>, 
                [<POSTCONDITION>, ...]], 
            [ <PRECONDITION>, 
                [<POSTCONDITION>, ...]], 
            ...],
    "new_skill_1": [
            [ <PRECONDITION>, 
                [<POSTCONDITION>, ...] ], 
            [ <PRECONDITION>, 
                [<POSTCONDITION>, ...]], 
            ...],
    ...}
```
\end{lstlisting}
The response follows the grammar:
\begin{scriptsize}
\begin{verbatim}
<new_skill>: [<intermediate_transition>+]
<intermediate_transition> = [<precondition>, 
                            [<postcondition>+]]
<precondition> = [<controllable_input>+]
<postcondition> = [<controllable_input>+]
\end{verbatim}
\end{scriptsize}

Each pre or post-condition in the new skills should be a complete controllable input state.
Do not include original skills in the new skills. 
Do not include any comments in skills.
\textbf{\textless New skill candidates to be returned here\textgreater}
    \end{tcolorbox}
% \vspace{-1.5em}
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % New skills that fail safety analysis
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \begin{tcolorbox}[
%       colback=red!5,       % second color (red)
%       colframe=red!75,
%       width=\textwidth,
%       boxrule=0.5pt,
%       sharp corners
%     ]
% \scriptsize\textbf{F. Example new skill candidates that violate safety constraints.}
% \begin{lstlisting}[basicstyle=\tiny]
% ```JSON
% {    "new_skill_0": [
%         [["p_base_x2", "p_cup_ee"],
%         [["p_base_x3", "p_cup_ee"]]],
%         [["p_base_x3", "p_cup_ee"],
%         [["p_base_x4", "p_cup_ee"]]]]}
% ```
% \end{lstlisting}
% \textbf{Feedback from safety analysis}: 
% new\_skill\_0 violates the hard constraints 
% $\square \neg (\bigcirc \varol{\textrm{base}}{x_3} \land \bigcirc \varol{\textrm{cone}}{x_3})$.
% % "!(p\_base\_x3' \& p\_cone\_x3')"
%     \end{tcolorbox}
    \vspace{-1.5em}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % New skills that fail safety analysis
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{tcolorbox}[
      colback=red!5,       % second color (red)
      colframe=red!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
\scriptsize\textbf{F. Example new skill candidates that violate safety constraints.}
\begin{lstlisting}[basicstyle=\scriptsize]
```JSON
{    "new_skill_0": [
        [["p_base_x2", "p_cup_ee"],
        [["p_base_x3", "p_cup_ee"]]],
        [["p_base_x3", "p_cup_ee"],
        [["p_base_x4", "p_cup_ee"]]]]}
```
\end{lstlisting}
\textbf{Feedback from safety analysis}: 
new\_skill\_0 violates the hard constraints 
$\square \neg (\bigcirc \varol{\textrm{base}}{x_3} \land \bigcirc \varol{\textrm{cone}}{x_3})$.
% "!(p\_base\_x3' \& p\_cone\_x3')"
    \end{tcolorbox}
% \vspace{-1.5em}

  \end{minipage}
  
  \caption{\textbf{Case study for Example~\ref{example:1}}. 
  % We study a violation described in Section V.C. of 
  % our previous work
  % \cite{meng2024automated}. 
  % We omit the description here for space.
  % The left column 
  (A)-(D) 
  describe
  the prompts and 
  LLM responses from informalization.
  % The right column 
  (E)-(G)
  present the
  repair prompt and 
  two sets of new skill candidates from \gls{llms},
  along with the feedback from formal analyses.
  % In the prompt,
  We use \textrm{p\_object\_region}
  to represent the input $\varol{\textrm{object}}{\textrm{region}}$ \hkc{in all of these, what is the actual prompt or feedback provided to the LLM? not the ltl symbols, the actual text? it is ok to add the text in $< >$ for space reasons, but the rest should be EXACTLY what the prompt and response were}
  \qm{It is exactly the prompt and response except that I change the symbols from p\_object\_region to $\varol{object}{region}$ for better visual presentation (otherwise it looks quite ugly). I can also change them back if needed. }
%
  }
  \label{fig:casestudy}
  \vspace{-0.25in}
\end{figure*}



==> figures/casestudy_backup.tex <==
% \begin{figure*}[ht]
%   \centering
%   % Scale the entire content to 80% of the text width:
%   \resizebox{\textwidth}{!}{%
%     \begin{tabular}{c}
%       % --- First row: Two boxes side by side ---
%       \begin{tabular}{cc}
%         % Left box
%         \begin{minipage}{0.45\textwidth}
%           \begin{tcolorbox}[colback=blue!5!white, colframe=mybrown!75!black]
%           \scriptsize
%             \textbf{LLM Response:}\\[1mm]
%             Each input proposition $\varol{o}{r}$ represents the condition that object $o$ is located within region $r$. The grounding function $\grounding$ maps each proposition $\varol{o}{r}$ to the set of physical states where the pose of object $o$ is in region $r$.
%           \end{tcolorbox}
%         \end{minipage}
%         &
%         % Right box
%         \begin{minipage}{0.45\textwidth}
%           \begin{tcolorbox}[colback=green!5!white, colframe=red!75!black]
%             \textbf{Additional Info:}\\[1mm]
%             Here you can include further details or another response.
%           \end{tcolorbox}
%         \end{minipage}
%       \end{tabular}\\[2ex] % End of first row with extra vertical spacing
%       % --- Second row: One box spanning most of the width ---
%       \begin{minipage}{0.9\textwidth}
%         \begin{tcolorbox}[colback=yellow!5!white, colframe=blue!75!black]
%           \textbf{Further Details:}\\[1mm]
%           Additional explanatory text or extended information can go here.
%         \end{tcolorbox}
%       \end{minipage}\\[2ex]
%       % --- Third row: Two boxes side by side ---
%       \begin{tabular}{cc}
%         % Left box
%         \begin{minipage}{0.45\textwidth}
%           \begin{tcolorbox}[colback=purple!5!white, colframe=black!75!black]
%             \textbf{Conclusion:}\\[1mm]
%             Concluding remarks or summaries.
%           \end{tcolorbox}
%         \end{minipage}
%         &
%         % Right box
%         \begin{minipage}{0.45\textwidth}
%           \begin{tcolorbox}[colback=red!5!white, colframe=orange!75!black]
%             \textbf{Notes:}\\[1mm]
%             Some additional notes or observations.
%           \end{tcolorbox}
%         \end{minipage}
%       \end{tabular}
%     \end{tabular}
%   }
%   \caption{A figure spanning two columns with a mix of horizontal and vertical stacking of \texttt{tcolorbox} environments.}
%   \label{fig:stacked-tcolorboxes}
% \end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \documentclass[twocolumn]{article}
% \usepackage[most]{tcolorbox}
% \usepackage{xcolor}
% \usepackage{graphicx}

\begin{figure*}[ht]
  \centering
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Top row: abstraction informalization
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  \begin{minipage}[t]{0.496\textwidth}
    \begin{tcolorbox}[
      colback=blue!5!white,      % first color (blue)
      colframe=blue!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
    \scriptsize\textbf{Abstraction informalization prompt.} \\%\\[1mm]
    % \textbf{System prompt:}
You are a researcher in robotics and an expert in formal methods for robotics.
% \textbf{User prompt:}
% \vspace{-1.5em}
You are given an abstraction that contains a set of input propositions $\inp$, 
a physical state space $\ps \subseteq R^n$, 
and a grounding function $\grounding: \inp \to 2^\ps$ that maps each input proposition to a set of physical states. 
You are asked to explain the physical meaning of the input propositions.

\# Input propositions: 
\textbf{\textless Inserted input propositions \textgreater}

\# Grounding: 
\textbf{\textless Inserted grounding function \textgreater}

Please only provide a concise, general explanation covering all input propositions' physical meaning. Do not provide any examples.

\textbf{\textless Informalized abstraction to be inserted here\textgreater}
    \end{tcolorbox}
  \end{minipage}
  %
  %
  %
  \hfill
  %
  %
  %
  \begin{minipage}[t]{0.496\textwidth}
    \begin{tcolorbox}[
      colback=red!5,       % second color (red)
      colframe=red!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
    \scriptsize\textbf{Example informalized abstraction.} \\%\\[1mm]
    Each input proposition $\varol{o}{r}$ represents the condition that object $o$ is located within region $r$. The grounding function $\grounding$ maps each proposition $\varol{o}{r}$ to the set of physical states where the pose of object $o$ is in region $r$. The proposition $\varol{\textrm{empty}}{}$ signifies the status of the cup, indicating whether it is empty.
    \end{tcolorbox}
  \end{minipage}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Second row: strategy informalization
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  \begin{minipage}[t]{0.496\textwidth}
    \begin{tcolorbox}[
      colback=blue!5!white,      % first color (blue)
      colframe=blue!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
    \scriptsize\textbf{Strategy informalization prompt.} \\%\\[1mm]
    You are a researcher in robotics and an expert in formal methods for robotics.
You are given an abstraction of the environment, a set of robot skills, a GR(1) specification, and its corresponding synthesized strategy. You are asked to describe the behavior of the strategy. I will first give an example of a strategy, its behavior description, and its explanation. Then, I will ask you to describe the behavior of a different strategy.

\# Example: \\
\#\# Input propositions: 
$["a"]$\\
\#\# Output propositions: 
$["b"]$\\
\#\# Task specification: 
$a \to b \land \square \lozenge (a\to b) \land \square \lozenge (\neg a\to \neg b)$\\
\#\# Strategy:
\{"nodes": \{"0": \{"rank": 0, "state": ["a"], "trans": [1, 2]\}, "1": \{"rank": 0, "state": [], "trans": [1, 0]\}, "2": \{"rank": 0, "state": ["a", "b"], "trans": [1, 0]\}\}\}\\
\#\# Behavior:
Initially, the input 'a' is true and the output 'b' is false. If 'a' remains true, 'b' turns on and off repeatedly. While 'a' becomes false, 'b' remains false.\\
\#\# Explanation:
"Initially, the input 'a' is true and the output 'b' is false" corresponds to node 0. "If 'a' remains true, 'b' turns on and off repeatedly" corresponds to the transitions between node 0 and node 2. "While 'a' becomes false, 'b' remains false" corresponds to the transitions from node 0 and node 2 to node 1 and self-transitions to node 1.

\# Problem:
Now, I will ask you to describe the behavior of a different strategy. You are given: (1) an abstraction of the physical workspace and objects in the workspace, (2) a set of robot skills, (3) a task specification, and (4) a synthesized robot controller.

\#\# Input propositions:
\textbf{\textless Inserted inputs and informalized abstraction\textgreater}

\#\# Output propositions:
\textbf{\textless Inserted output propositions\textgreater}

\#\# Task specification:
We use the \gls{gr1} fragment of Linear Temporal Logic to encode the task specification. The task specification is given in the following JSON file:
\textbf{\textless Inserted task specification \textgreater}

\#\# Strategy:
We represent the robot strategy synthesized from the specification as a finite state automaton. 
For each node, 'rank' represents which liveness goal the node is trying to satisfy, 'state' represents the value of each variable in the state, in the order of the field 'variables', and 'trans' represents the possible successor states. 
The strategy is in the following JSON file:
\textbf{\textless Inserted strategy\textgreater}

Please describe the behavior of the synthesized strategy only. Do not provide any explanation:
\textbf{\textless Informalized strategy behavior to be inserted here\textgreater}
    \end{tcolorbox}
  \end{minipage}
  %
  %
  %
  \hfill
  %
  %
  %
 
%
  %
  %
  \hfill
  %
  %
  %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Third row: repair 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  \begin{minipage}[t]{0.496\textwidth}
    \begin{tcolorbox}[
      colback=blue!5!white,      % first color (blue)
      colframe=blue!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
    \scriptsize\textbf{Repair prompt.} \\%\\[1mm]
    You are a researcher in robotics and an expert in formal methods for robotics.\\
\textbf{User prompt:}
You are given: (1) an abstraction of the physical workspace and objects in the workspace, (2) a set of robot skills, (3) a task specification, (4) the original behavior of the synthesized strategy, and (5) a violated observation during the robot execution.
You are asked to provide a set of new skills that along with the original skills can allow the robot to recover from the violation and satisfy the task specification.

\# Abstraction:\\
\#\# Input propositions:
\textbf{\textless Inserted inputs and informalized abstraction description\textgreater}

\#\# Output propositions:
\textbf{\textless Inserted output propositions\textgreater}

\# Task specification:\\
We use the \gls{gr1} fragment of Linear Temporal Logic to encode the task specification. The task specification is given in the following JSON file:
\textbf{\textless Inserted task specification \textgreater}

\# Strategy behavior:
\textbf{\textless Inserted informalized strategy behavior description\textgreater}

\# Assumption Violation:
During the robot execution, we detect that an observed transition violates some environment safety assumptions.

The violated observation is in the following JSON file:\\
\textbf{\textless Inserted assumption violation $t=(\inpstate, \outstate, \inpstateprime)$ \textgreater}

The violated environment safety assumptions are as follows:\\
\textbf{\textless Inserted violated assumptions \textgreater}

\# Returns:
After the assumption violation, we relax the violated assumption to include the observed violation transition. You are asked to provide a set of new skills that, along with the original skills, allow the robot to continue satisfying the task after the assumption violation.
Please respond with new skills only in the following format:
\begin{lstlisting}
```JSON
{    
    "new_skill_0": [
            [ <PRECONDITION>, 
                [<POSTCONDITION>, ...]], 
            [ <PRECONDITION>, 
                [<POSTCONDITION>, ...]], 
            ...],
    "new_skill_1": [
            [ <PRECONDITION>, 
                [<POSTCONDITION>, ...] ], 
            [ <PRECONDITION>, 
                [<POSTCONDITION>, ...]], 
            ...],
    ...
}
```
\end{lstlisting}

The response follows the grammar:
\begin{verbatim}
<new_skill>: [<intermediate_transition>+]
<intermediate_transition> = [<precondition>, [<postcondition>+]]
<precondition> = [<controllable_input>+]
<postcondition> = [<controllable_input>+]
\end{verbatim}

Each pre or post-condition in the new skills should be a complete controllable input state.
Do not include original skills in the new skills. 
Do not include any comments in skills.

\textbf{\textless New skills to be returned here\textgreater}
    \end{tcolorbox}
  \end{minipage}
 
  \begin{minipage}[t]{0.496\textwidth}
    \begin{tcolorbox}[
      colback=red!5,       % second color (red)
      colframe=red!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
    \scriptsize\textbf{Example informalized strategy.} \\%\\[1mm]
    The synthesized strategy behaves as follows:
Initially, the robot's base is at position $x_4$, the cup is at location $k_2$, the block is at location $k_1$, the cone is at $x_3$, the plate is at $k_0$, and the cup is empty.

When the cup becomes **not empty**, the robot executes **skill4** to pick up the block from $k_1$ and then **skill7** to place the block at $k_3$. Next, the robot uses **skill2** to pick up the cup from $k_2$. It then executes **skill1** to move from $x_4$ via $x_2$ to $x_0$ while holding the cup. At $x_0$, the robot uses **skill6** to place the cup on the table.

When the cup becomes **empty** again, the robot executes **skill3** to pick up the cup from the table. It then uses **skill0** to move from $x_0$ via $x_2$ to $x_4$ while holding the cup. At $x_4$, the robot executes **skill5** to place the cup back at $k_2$.
    \end{tcolorbox}
  \end{minipage}

  


  % Bottom row: one box spanning full width
  \begin{minipage}[t]{\textwidth}
    \begin{tcolorbox}[
      colback=green!5,     % third color (green)
      colframe=green!75,
      width=\textwidth,
      boxrule=0.5pt,
      sharp corners
    ]
    \scriptsize\textbf{Box 3} %\\[1mm]
    Content for the third box goes here.
    \end{tcolorbox}
  \end{minipage}
  
  \caption{A two-column layout with three aligned boxes using three colors.}
  \label{fig:aligned-boxes}
\end{figure*}




==> figures/grammar.tex <==
\begin{figure}[t]
  \centering
  \begin{minipage}{\columnwidth}
    \lstset{
      basicstyle=\ttfamily\scriptsize,
      breaklines=true,
      frame=single,
      xleftmargin=0pt,
        framexleftmargin=0pt,
        xrightmargin=0pt,
        framexrightmargin=0pt
    }
    \begin{lstlisting}
    <new_skill>: [<intermediate_transition>+]
    <intermediate_transition> = [<precondition>, 
                                [<postcondition>+]]
    <precondition> = [<controllable_input>+]
    <postcondition> = [<controllable_input>+]
    \end{lstlisting} 
  \end{minipage} 
  \caption{Grammar of new skills.} \label{fig:skill_grammar} 
\end{figure}
